NeRF Revisited: Fixing Quadrature Instability in Volume Rendering

Neural radiance fields (NeRF) rely on volume rendering to synthesize novel views. Volume rendering requires evaluating an integral along each ray, which is numerically approximated with a finite sum that corresponds to the exact integral along the ray under piecewise constant volume density. As a consequence, the rendered result is unstable w.r.t. the choice of samples along the ray, a phenomenon that we dub quadrature instability. We propose a mathematically principled solution by reformulating the sample-based rendering equation so that it corresponds to the exact integral under piecewise linear volume density. This simultaneously resolves multiple issues: conflicts between samples along different rays, imprecise hierarchical sampling, and non-differentiability of quantiles of ray termination distances w.r.t. model parameters. We demonstrate several benefits over the classical sample-based rendering equation, such as sharper textures, better geometric reconstruction, and stronger depth supervision. Our proposed formulation can be also be used as a drop-in replacement to the volume rendering equation of existing NeRF-based methods. Our project page can be found at pl-nerf.github.io.

==> sections/0-abstract_old.tex <==
\vspace{-0.4cm}
\begin{abstract}
  %\mika{}, \guandao{}, \leo{}
  \vspace{-0.2cm}
  Neural radiance fields (NeRF) rely on volume rendering to synthesize novel views. Volume rendering requires evaluating an integral along each ray, which is numerically approximated with a finite sum that corresponds to the exact integral along the ray under piecewise constant volume density. As a consequence, the rendered result is unstable w.r.t. the choice of samples along the ray, a phenomenon that we dub \emph{quadrature instability}. We propose a mathematically principled solution by reformulating the sample-based rendering equation so that it corresponds to the exact integral under piecewise linear volume density. This simultaneously resolves multiple issues: conflicts between samples along different rays, imprecise hierarchical sampling, and non-differentiability of quantiles of ray termination distances w.r.t. model parameters. We demonstrate several benefits over the classical sample-based rendering equation, such as sharper textures, less fuzzy surfaces, and stronger depth supervision. 
\end{abstract}
  \vspace{-0.2cm}

==> sections/1-introduction_old.tex <==
  \vspace{-0.3cm}
\section{Introduction}\label{sec:intro}
  \vspace{-0.2cm}
The advent of neural radiance fields (NeRF)~\cite{mildenhall2020nerf} has sparked a flurry of work on neural rendering and has opened the way to many exciting applications~\cite{chen2022mobilenerf,Li20arxiv_nsff,hedman2021snerg,park2021hypernerf}. One of the key underpinnings of NeRF is volume rendering~\cite{max1995optical} -- it is especially well-suited to end-to-end differentiable rendering~\cite{Kato2020DifferentiableRA}, since the rendered image is a smooth function of the model parameters. This has made it possible to learn the 3D geometry and appearance solely from a loss on rendered images w.r.t. the real observed images. 

In volume rendering, the rendered colour $\hat{y}$ for every pixel is an expectation of the colours along the ray cast through the pixel w.r.t. the distribution over ray termination distance $s$~\cite{kangle2021dsnerf}. 
\begin{equation}
\hat{y} = \mathbb{E}_{s\sim p(s)}[c(s)] = \int_0^\infty p(s)c(s) \,\dif s
\label{eq:continuous_volume_rendering}
\end{equation}
where $p(s)$ denotes the probability density function (PDF) of the distribution over ray termination distance $s$ and $c(s)$ denotes the the colour as a function of different points along the ray. 

In general, $p(s)$ and $c(s)$ can be of arbitrary forms, so evaluating this integral analytically is not possible. Therefore, in practice, $\mathbb{E}_{s\sim p(s)}[c(s)]$ is approximated with quadrature. The quadrature formula that is most commonly used in the NeRF literature takes the following form:

\begin{equation}
\mathbb{E}_{s\sim p(s)}[c(s)] = \sum_{j=0}^{N} T_j \paren{1 - e^{-\tau_j(s_{j+1}-s_j)}}c_j,
\label{eq:constant_volume_rendering}
\end{equation}
where $T_j = \exp\Big(-\sum_{k=0}^j -\tau_k(s_{k+1}-s_k)\Big)$ and $\tau_k$ is the opacity evaluated at a sample $s_k$ along the ray. 

This expression is derived from the exact integral under a piecewise constant approximation to the opacity and colour along the given ray~\cite{max1995optical}. 

However, this seemingly simple, innocuous approximation can result in the rendered image being sensitive to the choice of samples along the ray at which the opacity $\sigma(s)$ and colour $c(s)$ are evaluated. While this does not necessarily cause a practical issue in classical rendering pipelines~\cite{max1995optical, max_et_al:DFU:2010:2709, levoy1990efficient}, it has surprising consequences when it is used in a neural rendering context. Specifically, because the opacity at all points within the interval between two samples is assumed to be the same, there is a band near the surface of the geometry where opacity at all points within the band is as high as points on the surface itself. Because different rays cast from the cameras can pass through this band at different angles and offsets, both the number and the positions of samples within this band can be very different across different rays. As a result, simultaneously supervising these rays to produce the same colour values as in the real image captures can give rise to conflicting supervisory signals, which can result in artifacts like fuzzy surfaces and blurry texture. 

Moreover, because the piecewise constant approximation gives rise to a closed form expression that is equivalent to an expectation w.r.t. a discrete random variable, it is common practice in the NeRF literature to draw samples along the ray from the discrete distribution~\cite{mildenhall2019llff}. This is commonly used to draw importance samples, and also to supervise the samples along the ray~\cite{uy-scade-cvpr23}, for example in losses that penalize deviation of the samples from the true depth~\cite{deng2022depth}. Sampling from the discrete distribution requires the definition of a continuous surrogate function to the cumulative distribution function (CDF) of the discrete random variable, which unfortunately yields imprecise samples. As a result, samples that are drawn may not be close to the surface even if the underlying probability density induced by the NeRF is concentrated at the surface. Additionally, individual supervision cannot be provided to each sample drawn from the surrogate, because the gradient of the loss w.r.t. each sample would be almost zero everywhere. 

We dub this problem \emph{quadrature instability}. In this paper, we revisit the quadrature used to approximate volume rendering in NeRF and devise a different quadrature formula~\cite{max1995optical} based on a different approximation to the opacity. While one way to improve the robustness of quadrature to the choice of samples is to consider piecewise linear approximations to both the opacity and colour, it is known from the classical volume rendering literature~\cite{williams1992volume} that this unfortunately leads to a dead end: the analytical form of the integral under this approximation is an unwieldy expression that is numerically unstable and computationally expensive to evaluate. 

Is there a way around this? In this paper, we discover that when we consider a piecewise \emph{linear} approximation to the opacity and piecewise \emph{constant} approximation to the colour, the resulting integral is a simple closed-form expression that can be evaluated efficiently and stably. We leverage this finding to design a new quadrature method for volume rendering in NeRFs and demonstrate reduced artifacts and improved rendering quality. We also devise a new way to sample directly from the distribution of samples along each ray induced by NeRF without going through the surrogate, which opens the way to a more refined importance sampling approach and a more effective method to supervise samples using depth. 

\vspace{-0.2cm}
%This can result in two different rays 
%conflicting supervision



%volume rendering is embedded within the loss function for learning 3D scene representations. 



%\begin{itemize}


    %\item Recently, there has been an explosion of works on neural fields ranging from applications such as novel view synthesis, 3D reconstruction, etc, as they are able to produce high quality results due to the inductive smoothness of neural networks (by model construction).
    %\item The crux of being able to learn a neural field is the differentiability of the loss function, which is enabled by the volumetric rendering equation. (Not sure how to make this rendering specific, since for volumetric rendering we are saying we only have a loss on images, ie no 3D model as in SDF).
    %\item This allowed for end-to-end training with only using 2D image-based losses that led to the popularity and versatile usability of NeRFs (idk how to disentangle the equation from NeRF, especially since we are dealing with opacity).
    %\item The volumetric rendering equation consists of a continuous integral, which is discretized into bins with ray samples and integrated using numerical quadrature. What is overlooked by previous works is that each bin is assumed to be constant -- ie the integral along the ray is assumed to be piecewise constant.
    %\item This poses problems such as discretization errors (not sure how to write it that approximating as linear is better than constant from a mathematical perspective), rays conflicting? multiple solutions for the surface in the bin? ... Sorry this is rough.
    %\item In this work, we rewrite the volumetric rendering equation with a piecewise linear assumption for opacity, that derives into a simple expression for numerical quadrature.
    %\item We show that this the linear formulation allows us to derive an analytical closed-form expression for the surface on the bin. This results into solving a quadratic equation by considering the probability distribution on ray termination, where we theoretically prove always has one unique solution -- (hierarchical sampling part: we prove that the solution always exists and is unique). This allows us to optimize for better samples/cleaner surface without conflicts such as in the constant case.
    %\item Moreover, we show that we can analytically also derive the exact gradient at the 3D samples (because we can write out the probability distribution) that allows us to accurate supervise with depth.
    %\item Experiments show that our piecewise linear approach allows for 1) better novel view synthesis especially under the setting of  different camera distances (hence having conflicting rays), 2) better geometry/depth recovery due to the correct gradient/depth supervision (this cover both the scaled gradient and the binning error in constant), and 3) better/faster voxel-based neural field training allowing for fewer samples due to analytical integration.
    %(And/or if SCADE-like setup can work, then applications to real data / in-the-wild environments).
%\end{itemize}

% \mika{In general, I think we need to also be clear here that we rewrote it for opacity. Not sure if saying it's rewriting the "volumetric rendering equation" is accurate, since that might imply the integration with color. Also we might need to bring up MipNeRF here and differentiate clearly if I can't get the experiments out.}

==> sections/2-relatedworks_old.tex <==
\section{Related Work}
\vspace{-0.3cm}
\paragraph{NeRFs.} Neural Radiance Field (NeRF) is a powerful representation for novel-view synthesis~\cite{mildenhall2020nerf} that represents a scene using the weights of an MLP that is rendered by volumetric rendering~\cite{max1995optical}. A key finding to the success of NeRF was the use of positional encoding~\cite{tancik2020fourier, vaswani2017attention} to effectively increase the capacity of the MLPs that models the opacity and emitted color as a function of a 3D coordinate and viewing direction. Many works extend NeRF such as handling larger or unbounded scenes~\cite{Zhang2020NeRFpp,barron2022mip360,xiangli2022bungeenerf,tancik2022block}, unconstrained photo collections~\cite{martinbrualla2020nerfw}, dynamic and deformable scenes~\cite{li2021neural, park2021nerfies} and sparser input views~\cite{deng2022depth,yu2021pixelnerf,wang2021ibrnet, uy-scade-cvpr23, yuan2022neural}. Other works include faster training and inference time~\cite{hedman2021bake-nerf,reiser2021kilonerf,yu2021plenoctrees} as well as model compression~\cite{Chen2022ECCV}. There are a number of papers that aim to improve the rendering quality of NeRF. Some do so by utilizing different kinds of supervision such as NeRF in the Dark~\cite{mildenhall2022rawnerf}, while others tackle this by improving the model~\cite{barron2021mipnerf, barron2023zipnerf}. MipNeRF~\cite{barron2021mipnerf} changes the model input by introducing integrated positional encoding (IPE) to reduce the aliasing effect along the xy coordinates. ZipNeRF~\cite{barron2023zipnerf} modifies the proposal network to a grid enabling it to be used together with IPE. In contrast, our work focuses on changing the objective function by modifying the rendering equation from piecewise constant opacity to piecewise linear, while keeping the model and supervision fixed. Additionally, ZipNeRF~\cite{barron2023zipnerf} also brings up a model specific issue on z-aliasing, where their model struggles under this setting. Similar to z-aliasing observed by ZipNeRF, we consider the setting of having conflicting supervision when presented with training views at different distances from the scene. While they may appear similar on the surface, the phenomena we study is different in that it is general and independent of the model, on having conflicting ray supervision from camera views, e.g. different camera-to-scene distances and the grazing angle setup.
\vspace{-0.3cm}
% Our work is focused on a general phenomena, independent of the model, on having conflicting supervision on rays cast from cameras at different distances or angles from the scene. 

\paragraph{Importance Sampling on NeRFs.} Densely sampling and evaluating NeRF along multiple points in each camera ray is inefficient. Inspired by an early work on volume rendering~\cite{levoy1990efficient}, prior works typically use a coarse-to-fine hierarchical sampling strategy where the final samples are obtained by importance sampling of a coarse proposal distribution~\cite{mildenhall2020nerf,barron2021mipnerf,barron2022mip360,hedman2021bake-nerf}. These importance samples are drawn using inverse transform sampling where a sample is obtained by taking the inverse of the cumulative density function (CDF) of the proposal ray distribution. However, prior NeRF works that assume piecewise constant opacity result in a non-invertible CDF, and instead introduce a surrogate invertible function derived from the CDF in order to perform importance sampling. In contrast, our work that utilizes a piecewise linear opacity assumption results in an invertible CDF and a closed-form solution to obtain samples with inverse transform sampling. Other works also attempt to alter sampling using neural networks or occupancy caching~\cite{wang2021ibrnet,sun2022dvgo,sun2022dvgoi,liu2020neural}.
These techniques are orthogonal to our work as they propose changes to the model as opposed to our work where importance sampling is derived from a given model.
\vspace{-0.3cm}
% To handle samples along the ray direction, prior works usually use coarse-to-fine hierarchical sampling techniques, where the final samples are obtained by importance sampling of a coarse proposal distribution~\cite{mildenhall2020nerf,barron2021mipnerf,barron2022mip360,hedman2021bake-nerf}.
% These works assume the coarse proposal distribution to be piece-wise constant, which makes it difficult to optimize the coarse distribution during hierarchical sampling.
% Our approaches replace the piece-wise constant interpolation with a piece-wise linear one, allowing us to create more accurate hierarchical samples and achieve better optimization.
% Some other works attempt to alter the sampling using neural networks or occupancy caching~\cite{wang2021ibrnet,sun2022dvgo,sun2022dvgoi,liu2020neural}.
% These techniques are orthogonal to our proposed piece-wise linear formulation.

% \paragraph{NeRFs.}
% Neural Radiance Fields (NeRF) are a powerful representation for novel-view synthesis~\cite{mildenhall2020nerf}.
% Tremendous research has been done to make NeRF better, such as scaling to larger or unbounded scene~\cite{Zhang2020NeRFpp,barron2022mip360,xiangli2022bungeenerf,tancik2022block}, faster training and inference~\cite{liu2020neural,lindell2021autoint,reiser2021kilonerf,lombardi2021mixture,sitzmann2021light,chen2022tensorf,yu_and_fridovichkeil2021plenoxels}, reducing the amount of supervision~\cite{deng2022depth,yu2021pixelnerf,wang2021ibrnet} and adapting to dynamic scenes~\cite{xian2021space,Li20arxiv_nsff,Park20arxiv_nerfies,Pumarola20arxiv_D_NeRF}.
% Laying at the foundation of these works is the differentiable volume rendering equation, which is this paper's key subject of interest.
% To render an image, NeRFs need to integrate the radiance along the frustum of the pixel using discrete samples, which can lead to aliasing artifacts if not done properly~\cite{nyquist1928certain,shannon1949communication}.
% Recent works developed techniques to avoid aliasing in the spatial domain by pre-filtering the radiance fields and multi-sampling~\cite{barron2023zipnerf,barron2021mipnerf,barron2022mip360,isaac2022exact-nerf,lindell2022bacon,yang2022pnf}.
% However, these works mostly focus on reducing aliasing in image coordinates and neglect the potential aliasing effects created by sampling the ray direction.
% To handle samples along the ray direction, prior works usually use coarse-to-fine hierarchical sampling techniques, where the final samples are obtained by importance sampling of a coarse proposal distribution~\cite{mildenhall2020nerf,barron2021mipnerf,barron2022mip360,hedman2021bake-nerf}.
% These works assume the coarse proposal distribution to be piece-wise constant, which makes it difficult to optimize the coarse distribution during hierarchical sampling.
% Our approaches replace the piece-wise constant interpolation with a piece-wise linear one, allowing us to create more accurate hierarchical samples and achieve better optimization.
% Some other works attempt to alter the sampling using neural networks or occupancy caching~\cite{wang2021ibrnet,sun2022dvgo,sun2022dvgoi,liu2020neural}.
% These techniques are orthogonal to our proposed piece-wise linear formulation.

\paragraph{Volume rendering.}
Volume rendering is an important technique in various computer graphics and vision applications as explored in different classical works~\cite{levoy1990efficient,westover1989interactive,drebin1988volume,max1995optical}. These works include studying ray sampling efficiency~\cite{levoy1990efficient} and data structures, e.g. octree~\cite{samet1990design} and volume hierarchy~\cite{rubin19803} for coarse-to-fine hierarchical sampling. The crux behind volume rendering is the integration over the weighted average of the color along the ray, where the weights is a function of the volume density (opacity). Max and Chen~\cite{max1995optical, max_et_al:DFU:2010:2709} derive the volume rendering equation under the assumption of piecewise constant opacity and color, which NeRF~\cite{mildenhall2019llff} and its succeeding works use to learn their neural scene representation. However, the piecewise constant assumption results in rendering outputs that are sensitive to the choice of samples as well the non-invertible CDF introducing drawbacks to NeRF training. Following up on~\cite{max1995optical}, works also~\cite{williams1992volume}  derive the volume rendering equation under the assumption that both opacity and color are piecewise linear that yield unwieldy expressions that lead to numerical issues and/or are expensive to compute. Some earlier works on rendering unstructured polygonal meshes that attempt to use this model~\cite{williams1998high}, but it is in general not commonly used in practice due to the mentioned issues and hence has yet to be adopted into learning neural scene representations. In this work, we address both sets of issues that arise from the piecewise constant opacity and color and piecewise linear opacity and color by reformulating the volume rendering equation to assume piecewise linear opacity and piecewise constant color. Our derivation results in a simple and closed-form formulation to volume rendering making it suitable for NeRFs.

% Levoy~\cite{levoy1990efficient} study the challenge of sampling rays efficiently, 


% An important challenge of volume rendering is to sample the ray efficiently~\cite{levoy1990efficient}.
% Traditional methods adapt coarse-to-fine hierarchical sampling using data structures such as Octtree~\cite{samet1990design} and volume hierarchies~\cite{rubin19803}.
% Many voxel-based NeRFs models leveraged similar approaches to accelerate rendering and training~\cite{hedman2021bake-nerf,reiser2021kilonerf,yu2021plenoctrees}. 

% As the original volume rendering is usually applied to discretized representation such as polygon mesh or voxels, people have derived the analytical form of the integration for piece-wise linear opacity model~\cite{williams1992volume,williams1998high,moreland2004fast}.
% However, these analytical equations are challenging to compute efficiently, which makes them less used in common practice.
% When volume rendering was first applied to a neural field representation like NeRF, people usually fell back to the piecewise constant assumptions, possibly for compute efficiency.
% Most NeRF papers adapted the non-smooth piece-wise constant assumption to interpolate the opacity model, leading to various optimization issues described in Section~\ref{sec:intro}.
% In this paper, we derive a computable volume-rendering equation with a piece-wise linear opacity model.



==> sections/3-method_old.tex <==
\vspace{-0.2cm}
\section{Background}
\vspace{-0.2cm}
\subsection{Volume Rendering Review}
\vspace{-0.2cm}
\paragraph{Definitions.} In classical literature, the process of volume rendering~\cite{max_et_al:DFU:2010:2709} mapping a 3D field of optical properties to a 2D image
% ~\ke{do you mean mapping 3D field of optical properties to a 2D image?}, 
and the visual appearance is computed
% ~\ke{I think this part is exact, assuming exact integration} 
through the exact \emph{integration} of these optical properties along the viewing rays.
In this optical model, each point in space is an infinitesimal particle with a certain \emph{opacity} $\tau$ that emits varying amounts of light, represented as a scalar \emph{color} $c$, in all viewing directions.
% \leo{In tradional volume rendering there is also scattering -- which most NeRF works ignore, I think}. 
The opacity $\tau$ is the differential probability of a viewing ray hitting a particle -- that is for a viewing ray $\mathbf{r}(s) = \mathbf{o}+s\mathbf{d}$, where $\mathbf{o}$ is the view origin and $\mathbf{d}$ is the ray direction, the probability of ray $\mathbf{r}$ hitting a particle along an infinitesimal interval $\dif s$ is $\tau(\mathbf{r}(s))\dif s$. Moreover, the transparency $T_{\mathbf{r}}(s)$ is defined as the probability that the viewing ray $\mathbf{r}$ travels a distance $s$ from the view origin without terminating, i.e. without hitting any particles.
\vspace{-0.1cm}
\paragraph{Continuous probability distribution along the ray $\mathbf{r}$.} 
% \vspace{-0.2cm}
%% Define probability distribution
As illustrated by Max and Chen~\cite{max_et_al:DFU:2010:2709}, since the events of not hitting a particle between 0 to $s$ and hitting a particle between $s$ and $s+\dif s$ are independent, the probability of ray $\mathbf{r}$ terminating at distance $s$ is given by $\tau(\mathbf{r}(s))T_{\mathbf{r}}(s)$, where $T_{\mathbf{r}}(s) = \exp(-\int_0^s \tau(\mathbf{u})\dif u)$ is derived from the independent events of not hitting a particle from 0 to $s$ and from $s$ to $s + \dif s$. Hence the continuous probability density function (PDF) the ray ${\mathbf{r}}(s)$ that describes the likelihood of a ray terminating and emitting at $s$ is given by 
% \vspace{-0.1cm}
\begin{equation}
	p(s) = \tau(\mathbf{r}(s))T_{\mathbf{r}}(s),
	\label{eq:pdf_ray}
\end{equation}

\noindent where $s\in [0, \infty]$ is a point on the ray $\mathbf{r}$. For notational simplicity we omit $\mathbf{r}$ and write it as $p(s) = \tau(s)T(s)$.
\vspace{-0.1cm}
\paragraph{Volume Rendering as a Continuous Integral.}
% \vspace{-0.2cm}
%% Expected color
The observed color of the ray is then the expected value of the colors $c(s)$ of all particles $s$ along the ray weighted by the probability of hitting them.
% color $c(s)$ aggregated over its the probability density function, by taking the weighted average of the colors of the hit particles
% ~\ke{colours of all particles along the ray weighted by the probability of hitting them}. 
Mathematically, this results in the following continuous integral\footnote{Practically the integral is taken with near $s_n$ and far $s_f$ bounds.}:

\begin{equation}
\mathbb{E}_{s\sim p(s)}[c(s)] = \int_0^\infty p(s)c(s) \,\dif s = \int_0^\infty \tau(s)T(s)c(s) \,\dif s\,.
\label{eq:continuous_volume_rendering}
\end{equation}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.85\linewidth]{figures/grazing_angle_v4.pdf}
    \caption{\textbf{Ray Conflicts: Grazing Angle.} (Left) Illustration of conflicting ray supervision at the grazing under the piecewise constant opacity. For the constant setting, to render perpendicular rays (yellow) correctly, the model has to store the associated optical properties at a region in front of the surface as a sample takes the values of the left bin boundary. In the presence of a ray near the grazing angle, it will be crossing this region of high opacity (the gradient in front of the surface), associating it with conflicting opacity/color signals. (Middle) This results in fuzzier surfaces as shown along the side of the microphone as there is a conflict in ray supervision between the perpendicular and grazing angle rays. Our piecewise linear opacity assumption alleviates this issue and results in a clearer rendered view. (Right) As shown, the resulting PDF is peakier and the CDF is sharper for our linear setting, where the plotted distributions correspond to the ray from the marked pixel in red.}
    % Left shows the piecewise constant opacity assumption (vanilla NeRF model) assigning the object's surface to different depths depending on whether the queried ray is perpendicular or parallel to the surface. With piecewise linear opacity assumption, our model can linearly interpolate between the left and right bins to obtain an accurate estimation of the surface. The rightmost plots are the PDF and the CDF plots for the distribution of the ray termination distance of the ray shot in the direction of the red cross point on the microphone. Because of our model's piecewise linear assumption and the ability to model accurate object surface, our model's pdf is much more \textit{unimodal} than the vanilla model with piecewise constant assumption.}
    \label{fig:grazing_angle}
    \vspace{-0.7cm}
\end{figure}

\paragraph{Quadrature under Piecewise Constant Opacity $\tau$.}
%%Integral defined on samples
Since this integral cannot in general be evaluated analytically, it is approximated with quadrature.
% Since it is not possible to evaluate the integral analytically for general volume densities, numerical integration (quadrature) is needed.
% The continuous integral above is numerically estimated using quadrature through discrete samples
% ~\ke{I'd motivate this by saying that it is not possible to evaluate the integral analytically for general volume densities, and so numerical integration (quadrature) is needed}. 
Let $s_1, s_2, ..., s_N$ be $N$ (ordered) samples on the ray that define the intervals, where $I_j = [s_j, s_{j+1}]$ is the  $j^{\text{th}}$ interval, and $I_0 = [0, s_1], I_N = [s_N, \infty]$. The volume density for particles along the interval $I_j$ is then approximated under the assumption that opacity is constant along each interval, making it \emph{piecewise constant} along the ray~\cite{max_et_al:DFU:2010:2709}. That is, for all $j$ we have:

\vspace{-0.1cm}
\begin{equation}
\forall s \in [s_j, s_{j+1}], \tau(s) = \tau(s_j), 
\label{piecewise_constant_opacity}
\end{equation}

\noindent for brevity we denote $\tau(s_j) = \tau_j$, i.e. $\tau_j$ is the opacity for sample $s_j$. Under this piecewise constant opacity assumption, the volume rendering equation Eq.~\ref{eq:continuous_volume_rendering} then becomes as follows:

\begin{equation}
\mathbb{E}_{s\sim p(s)}[c(s)] = \sum_{j=0}^{N} P_j c_j = \sum_{j=0}^{N} \paren{\int_{s_j}^{s_{j+1} }\tau(u)T(u)\,\dif u} c_j = \sum_{j=0}^{N} T_j \paren{1 - e^{-\tau_j(s_{j+1}-s_j)}}c_j,
\label{eq:constant_volume_rendering}
\end{equation}

\noindent where $T_j = \exp\Big(-\sum_{k=0}^j -\tau_k(s_{k+1}-s_k)\Big)$. Here, color $c_j$ is also approximated to be constant along each interval $I_j$. $P_j$ is the probability of each interval, which is mathematically equivalent to the probability of the interval. Now, let us define the discrete random variable $\tilde{s} = \tilde{f}(s)$, where 
\begin{equation}
    \tilde{f}(x) = \begin{cases} s_0 & x \leq s_0 \\ s_j & s_j \leq x < s_{j+1} \text{ for all } j \in \{1,...,N-1\} \\ s_N & x > s_N \end{cases},
\end{equation}

which gives corresponding probability mass function $\tilde{P}(s)$
% $Y=y_1, ..., y_N$ and $y_k = \frac{s_{k+1}-s_k}{L}$, $L$ being the length of the ray.
Observe that the analytical expression of the integral Eq.~\ref{eq:constant_volume_rendering} turns out to be the same as taking the expectation w.r.t. the discrete random variable $\tilde{s}$, i.e. $\mathbb{E}_{s\sim p(s)}[c(s)] = \mathbb{E}_{\tilde{s}\sim \tilde{P}(s)}[c(\tilde{s})]$. This piecewise constant opacity assumption in the volume rendering equation is used in most, if not all, existing NeRF works. We recommend the reader to read~\cite{max_et_al:DFU:2010:2709} for more detailed derivations and our supplementary for a more thorough walkthrough.
\vspace{-0.2cm}
% $f(x) = \begin{cases} s_0 & x \leq s_0 \\ s_j & s_j \leq x < s_{j+1} \forall i \in \{1,\ldots,N-1\} \\ s_N & x > s_N \end{cases}$

% $F(x) = \begin{cases} 0 & x \leq s_0 \\ \sum_{k<j} p(s_k) & 1 \leq x < s_{j+1} \forall i \in \{1,\ldots,N-1\} \\ s_N & x > s_N \end{cases}$

% Under this discrete approximation, the continuous integral is then approximated by the Riemann sum resulting in the following sample-based rendering equation~\ke{Technically each term in a Riemann sum is only the integrand at a value within the interval multiplied by the interval length, so it's not a Riemann sum. Instead it's the exact integral assuming a piecewise constant volume density. So the approximation happens when defining the volume density, not when integrating. So I would define the approximated volume density (i.e., eq. (4)), and then derive the integral of that volume density.}:

% \begin{equation}
% \mathbb{E}_{s\sim p(s)}[c(s)] = \sum_{j=0}^{N} P_j c_j = \sum_{j=0}^{N} \Big( \int_{s_j}^{s_{j+1} }\tau(u)T(u)\dif u\Big) c_j
% \label{eq:reimann_volume_rendering}
% \end{equation}

% \ke{Need the piecewise constant approximation of colour for the above to  be true}
% %%Constant Assumption on 
% where $P_j$ is the probability mass function (PMF)~\ke{before speaking of a pmf, we need to define what the random variable is. Also we need to motivate why we have a discrete RV now, e.g, it turns out to be mathemtically equivalent to taking the expectation w.r.t. that discrete RV} of the $j^{\text{th}}$ interval and $c_j$ represents the interval's expected color. To evaluate $P_j$, a further approximation is then taken under the assumption that opacity is \textbf{\emph{constant}} along each interval, that is $\forall j$ we have:

% \begin{equation}
% \forall s \in [s_j, s_{j+1}], \tau(s) = \tau(s_j), 
% \label{piecewise_constant_opacity}
% \end{equation}

% \noindent for brevity we denote $\tau(s_j) = \tau_j $. This results in the following PMF for  the ray (from Eq.~\ref{eq:pdf_ray}):

% \begin{equation}
% P_j = T_j (1 - \exp(-\tau_j(s_{j+1}-s_j))), \text{where } T_j = \exp\Big(-\sum_{k=0}^j -\tau_k(s_{k+1}-s_k)\Big),
% \label{eq:PMF_constant}
% \end{equation}

% \noindent which can be plugged into Eq.~\ref{eq:reimann_volume_rendering} 
% This piecewise constant opacity assumption in the volume rendering equation is used in most, if not all, existing NeRF works. We recommend the reader to read~\cite{maxchen1998} for more detailed derivations. We also include a more thorough walkthrough in our supplementary.

%\noindent Plugging to equation Eq.~\ref{eq:reimann_volume_rendering}, this leads to the volume rendering equation as used in all recent NeRF works:
%
%\begin{equation}
%\mathbb{E}_{s\sim p(s)}[c(s)] = \sum_{j=0}^{N} P_j c_j = \sum_{j=0}^{N} \Big( T_j (1 - \exp(-\tau_j(s_{j+1}-s_j))\Big) c_j.
%\label{eq:discrete_volume_rendering}
%\end{equation}
%
%\mika{Do we need to bring up that this is what the original nerf used? I guess we have to raise the issues there. But this means we have to introduce and define NeRF first? The derivations are all volume rendering specific. Except when inverse transform sampling is brought up}

\subsection{Neural Radiance Fields.} 
\vspace{-0.2cm}
Following Max and Chen~\cite{max1995optical}, Mildenhall et.al.~\cite{mildenhall2020nerf} introduced neural radiance fields, a neural scene representation that uses the volume rendering equation under the piecewise constant opacity assumption for novel view synthesis.
A neural radiance field (NeRF) is a coordinate-based neural scene representation, where opacity $\tau^{\theta}: \mathbb{R}^3 \rightarrow \mathbb{R}_{\geq 0}$ and color $c^{\psi}:\mathbb{R}^3 \times \mathbb{S}^2 \rightarrow [0, 255]^3$ are predicted at each continuous coordinate by parameterizing them as a neural network. To train the neural network, 2D images are used as supervision where each viewing ray is associated with a ground truth color. Volume rendering allows for the 3D coordinate outputs to be aggregated into an observed pixel color allowing for end-to-end training with 2D supervision. The supervision signal are on the coordinates of the ray samples $s_1, ..., s_N$, 
% which are obtained in practice through stratified sampling~\cite{mildenhall2020nerf}, 
which updates the corresponding output opacity and color at those samples. NeRF uses a importance sampling strategy by drawing samples from the ray distribution from a coarse network to generate better samples for rendering of their fine network. To sample from a distribution, inverse transform sampling is needed, that is, one draws $u \sim U(0,1)$ then passes it to the inverse of a cumulative distribution (CDF), i.e. a sample $x = F^{-1}(u)$, where $F$ is the CDF of the distribution. Under the piecewise constant assumption, the CDF of the discrete random variable $\tilde{s}$ is given by:
\begin{equation}
    \tilde{F}(x) = \begin{cases} 0 & x \leq s_0 \\ \sum_{k<j} \tilde{P}(s_k) & 1 \leq x < s_{j+1} \text{ for all } j \in \{1,...,N-1\} \\ 1 & x > s_N \end{cases}.
    \label{eq:pwc_cdf}
\end{equation}

This CDF is however non-continuous and non-invertible. NeRF's approach to get around this is to define a surrogate invertible function $G$ derived from its CDF, concretely, $G(y) = \frac{y-s_{j-1}}{s_j-s_{j-1}}\tilde{F}(s_j) + \frac{s_{j}-y}{s_j-s_{j-1}}\tilde{F}(s_{j-1}), \text{where } y\in[s_{j-1},s_j]$. Then taking $x = G^{-1}(u)$. However, this does not necessarily result in the samples from the actual ray distribution $p(s)$ from the model. 
\vspace{-0.4cm}
% \mika{This does not necessarily result in samples from the model distribution.... p(s)
% is however, not mathematically equivalent to the actual predicted ray distribution of the model.}

% The importance samples are drawn using inverse transform sampling by inverting the function $G(y) = \frac{y-s_{j-1}}{s_j-s_{j-1}}s_j + \frac{s_{j}-y}{s_j-s_{j-1}}s_{j-1}, \text{where } y\in[\tilde{F}(s_{j=1}), \tilde{F}(s_j)]$ derived from from the cumulative density function (CDF) of the discrete random variable $\tilde{s}$:

% \begin{equation}
%     \tilde{F}(x) = \begin{cases} 0 & x \leq s_0 \\ \sum_{k<j} p(s_k) & 1 \leq x < s_{j+1} \forall j \in \{1,...,N-1\} \\ s_N & x > s_N \end{cases}
% \end{equation}
% \noindent where a sample $x = G^{-1}(u)$, for $u\sim U(0,1)$.

% unstable 
% This causes issues in at training time \mika{can I say it this way?} due to 
% Utilizing the volume rendering equation Eq.~\ref{eq:reimann_volume_rendering} allowed for end-to-end training due to its differentiability. Supervision is obtained through ground truth images
% volume rendering equation makes training differentiable
% bring up supervision with gt images, discretization, importance sampling. (problems are brough up here with illustration)

% \mika{Blurb:- under the piecewise constant assumption, the PMF of the vieweing ray is not continuous with the discretization into $N$ samples, i.e. it is discontinuous at the bin boundaries. 
% - this discontinuity under the discretization causes issues (with optimization too? I'm not sure how to phrase this argument) such as conflicting ray samples such as on surfaces with high frequency color changes (See Figure), and along rays near the grazing angle causing a cloud.
% - this is because under the piecewise constant assumption, there is no notion or information on where the exact surface is under the ray distribution (as it is being optimized).
% - this also results in a problem when importance sampling as a discontinuous PMF would lead to a discontinuous CDF, which makes inverse transform sampling erroneous. }

% - unfortunately there are properties that are associated with PWC that may not be desirable in the context of nerfs
% - we will illustrate and discuss each in the following sections
% - to alleviate these issue, we propose a
% piecewise linear assumption on opacity.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.85\linewidth]{figures/ray_conflicts_v4.png}
    \caption{\textbf{Ray Conflicts: Different Camera-to-Scene Distances.} (Left) We show rendered views of the chair scene from cameras at different distances from the object, where at all distances the rendered output for our linear assumption result in sharper texture than the constant case because of the latter's sensitivity to the choice of samples. We also highlight the instability of the resulting renders for the constant model as shown by the noisier texture of the middle view compared to the closer and further views. (Right) An illustration that moving the camera to different distances from the object result in different samples that lead to conflicts.}
    % Vanilla NeRFs with piecewise constant opacity assumption will fail to capture high-frequency details in the scene because nearby rays will be assigned to the same opacity bin and there obtain the same color. Piecewise linear opacity does not suffer from this issue as it can accurately predict the opacity peak by linearly interpolating between the two closest bins.}}
    \label{fig:conflicting_ray}
    \vspace{-0.6cm}
\end{figure}

\section{Drawbacks of Piecewise Constant Opacity $\tau$ in NeRFs}
\vspace{-0.2cm}
\label{sec:constant_issues}
Unfortunately, there are properties associated with the piecewise constant opacity formulation that may not be desirable in the context of NeRFs. First, it is sensitive to the choice of samples, i.e. sample positions $s$, along the ray, a phenomenon we dub as \textit{quadrature instability}. This quadrature instability is due to the assumption that all points in an interval take the opacity of the left bin (Eq~\ref{piecewise_constant_opacity}), making it sensitive to sample positions. As illustrated in Figure~\ref{fig:grazing_angle}, this would lead to \emph{ray conflicts} in optimizing a NeRF when you have rays that are directly facing, i.e. perpendicular to, the surface (yellow rays) and rays that are close to the grazing angle (red ray), i.e. parallel to, the object. To render the perpendicular rays correctly, vanilla NeRF has to store the optical properties (opacity and color) associated with the perpendicular rays at a point before its intersection with the surface. This creates inaccurate signals to the optimization process when NeRF renders the ray at a grazing angle, as it will cross multiple conflicting opacity/colors (illustrated by the blue gradient). The sample sensitivity issue also arises when having cameras at different distances from the object as illustrated in Fig.~\ref{fig:conflicting_ray}, as this would lead to shifted sets of samples, causing inconsistencies when rendering at different camera-to-object distances. Notice that the noise on the texture of the chair is different across different viewing distances, where the middle view has fewer artifacts compared to the closer and further views.

The second issue comes from the CDF $\tilde{F}$ being piecewise constant (Eq~\ref{eq:pwc_cdf}). This leads to two consequences. First, the piecewise constant assumption makes $\tilde{F}$ non-invertible, hence, as mentioned in the previous section, importance sampling needs to be performed via a surrogate function $G$. This results in uniformity across the samples within the bin - samples within a bin are assigned with equal probability, leading to imprecise importance samples. The second consequence comes from the fact that $\tilde{F}$ is not continuous, leading to an issue in training a NeRF that has a loss based on its samples. In other words, there will be a vanishing gradient effect when taking the gradient w.r.t. the samples, such an example of a sample-based loss used for NeRFs is depth~\cite{uy-scade-cvpr23}.
\vspace{-0.2cm}
% This results to imprecise samples as within a bin, e.g. $[s_j, s_{j+1}]$ there is no differentiation between the probability of drawing 

% % 1. sensity to sample positions -- ray conflicts : define this. supervising on both rays creates on conflict.
% 2. F is PWC --> 1. non-invertible (importance sampling needing suggorate G) 2. is not continuous : if you have a loss based on the samples, if you take gradient wrt samples you;ll have vanishing gradients. backpropagation/learning issue for the nerf. an example of sample-based losses is depth (cite scade).

% non-invertibility of F --> imprecise importance samples. no differentiation -- sampling uniformly in a bin. "within a bin there is no differentiation between the samples, end to end is the same probability" if we have new function G is does not necessarily give us the function from the distribution. if you don't want that, take out the G but it's not invertible so importance sampling cannot be done. Or --> recall that noninvertible F --> so define G --> results in uniformity in bin.

% -  as you change the parameters of the neural network, it doesnt necessarily change the pmf of the network because of the discrete RV


% NeRF~\cite{mildenhall2020nerf} and its succeeding works adapt the original volume rendering work~\cite{} that assume piecewise constant opacity. This assumption results in a non-continuous probability density function for the viewing ray, causing multiple issues~\ke{I would not list all the issues here at once, and instead talk about the mathematical properties one by one, e.g., sensitivity to changes in sample positions, non-invertibility, non-differentiability. Then for each property, talk about the practical implications, e.g., ray conflicts.} such as conflicts between samples from different rays, imprecise hierarchical sampling and non-differentiability of quantiles of ray termination distances w.r.t. model parameters. The root cause of these issues is the rendered result is unstable w.r.t. the choice of samples along the ray, a phenomenon that we dub \emph{quadrature instability}. Figure~\ref{} shows an illustrative example on conflicting samples from different rays, \mika{show chair example where color changes in high frequency, and explain.}, which is caused by quadrature instability due to the piecewise constant assumption because color and opacity are always taken from the left bin, hence leading to blurry textures. Moreover, the non-continuous probability density leads to imprecise hierarchical sampling which becomes a bigger issues on rays near the grazing angle, i.e. close to being parallel to the object surface \mika{please help with this phrasing.}. Figure~\ref{} \mika{drawing of grazing angle rays and how there will be a cloud.} shows an illustrative example - near the grazing angle, the imprecise samples will cause the probability density to peak at different coordinates resulting in a fuzzy and more clouding surface. Figure~\ref{} \mika{show the microphone pdf (constant vs linear)} as the probability density function for a ray hitting such a region where there are training rays close to the grazing angle, and as shown the PDF is less peaky leading to fuzzier outputs.

% \mika{Do we have to mention depth here. I am not sure how to put in depth into the method.}~\ke{depth is just the ray termination distance, i.e., the RV the probability density is over}
  \vspace{-0.2cm}
\section{A Piecewise Linear Derivation for Opacity $\tau$ in Volume Rendering}
\vspace{-0.3cm}
It turns out that these problems are alleviated under the piecewise linear assumption for opacity. Earlier works~\cite{williams1992volume,williams1998high} show that naively turning both opacity and color to be piecewise linear along the ray leads to numerical issues, is expensive to compute and contain expressions that are unwieldly and hard to implement, and hence has not been commonly used in practice. 
To get around this issue, we propose making opacity piecewise linear, while keeping color piecewise constant, and show that this yields a \emph{simple} and \emph{closed-form} expression for the integral in volume rendering. Concretely, we derive the volume rendering equation under the piecewise linear opacity and piecewise constant color along a viewing ray, and we also solve for the closed-form solution to inverse transform sampling from the ray distribution leading to precise importance sampling.
\vspace{-0.3cm}

% In this work, we show that it turns out the issues raised in Sec~\label{sec:constant_issues} and in earlier works~\cite{} are alleviated under the piecewise linear opacity and piecewise constant color assumption leading to a clean formulation to volume rendering. We derive the corresponding volume rendering equation under the piecewise linear opacity and piecewise constant color assumption along a viewing ray. Moreover, we also solve for the closed-form solution to inverse transform sampling from the corresponding ray distribution leading to precise importance sampling.

% turns out when we use a piecewise lienar assumption these problems are alleviated.
% -turns out naively turning both opacity and color to pwl (cite old papers) causes issues ... (motivate this). (say numerical issues, expensive to compute)

% turns out under the pwl opacity and pwc color, the expression is simple and alleviates the problems above.

% \mika{Where and how to we bring up the figure on the ray distribution for the mic? Being peakier. As well as the problems for the constant: conflicting rays, cloudy surface...}

% \mika{Also, how do we highlight that the resulting form is non-trivial? Ie not just a simple plug-in of the midpoint.}

\paragraph{Volume Rendering with Piecewise Linear Opacity.} 
\begin{wrapfigure}{r}{0.33\linewidth}
\vspace{-0.4cm}
\begin{center}
    \includegraphics[width=0.34\textwidth]{figures/density.png}
\end{center}
\vspace{-0.5cm}
\caption{Illustration of opacities $\tau$ along a ray under the piecewise constant (green) and piecewise linear(orange) assumptions.}
\vspace{-0.6cm}
\label{fig:density}
\end{wrapfigure}
We propose an elegant reformulation to the sample-based rendering equation that corresponds to the exact integral under \textbf{piecewise linear} opacity while keeping piecewise constant color leading to a simple and closed-form expression for the integral. That is, instead of piecewise constant opacity as in Eq~\ref{piecewise_constant_opacity}, we assume a linear opacity for each interval $I_j$. Concretely, for $s\in[s_j, s_{j+1}]$, where $\tau_j=\tau(s_j), \tau_{j+1}=\tau(s_{j+1})$, we have

% We propose a mathematically principled approach by reformulating the sample-based rendering equation so that it corresponds to the exact integral under \textbf{piecewise linear} volume density leading to a clean expression. Instead of piecewise constant opacity as in Eq~\ref{piecewise_constant_opacity}, we assume a linear opacity for each interval $I_j$. Concretely, for $s\in[s_j, s_{j+1}]$, we have~\ke{we should define $\tau_i$'s. Also maybe a figure contrasting the piecewise constant vs. piecewise linear volume density might be nice to have, in case people can't picture what $\tau(s)$ looks like.}

\begin{equation}
\tau(s) = \left(\frac{s_{j+1}-s}{s_{j+1}-s_j}\right)\tau_j +  \left(\frac{s-s_j}{s_{j+1}-s_j}\right)\tau_{j+1}.
\end{equation}


\noindent which is a linear function w.r.t. $s\in[s_j, s_{j+1}]$. Fig. \ref{fig:density} This results in the probability of each interval $I_j$ to be given as follows:

%\begin{equation}
%\small
%P_i = \int_{s_j}^{s_{j+1}}\tau(s)T(s)\dif s = \int_{s_j}^{s_{j+1}}\tau(s)\exp{(-\int_{0}^{s}\tau(u)\dif u)}\dif s = \int_{s_j}^{s_{j+1}}\tau(s)T(s_j)\exp{(-\int_{s_j}^{s}\tau(u)\dif u)}\dif s
%\end{equation}
%
%\begin{center}
%	\begin{align*}
%	P_i = \int_{s_j}^{s_{j+1}}\tau(s)T(s)\dif s = \int_{s_j}^{s_{j+1}}\tau(s)\exp{(-\int_{0}^{s}\tau(u)\dif u)}\dif s &=\int_{s_i}^{s_{i+1}}\tau(s)\exp{(-\int_{0}^{s_i}\tau(u)\dif u)}\exp{(-\int_{s_i}^{s}\tau(u)\dif u)}\dif s\\
%	&=\int_{s_j}^{s_{j+1}}\tau(s)T(s_j)\exp{(-\int_{s_j}^{s}\tau(u)\dif u)}\dif s = T(s_j)\int_{s_j}^{s_{j+1}}\tau(s)\exp{(-\int_{s_j}^{s}\tau(u)\dif u)}\dif s 
%%	P_i &= \int_{s_i}^{s_{i+1}}\tau(s)T(s)\di s\\
%%	&= \int_{s_i}^{s_{i+1}}\tau(s)\exp{(-\int_{0}^{s}\tau(u)\di u)}\di s\\
%%	&= \int_{s_i}^{s_{i+1}}\tau(s)\exp{(-\int_{0}^{s_i}\tau(u)\di u)}\exp{(-\int_{s_i}^{s}\tau(u)\di u)}\di s\\
%%	&= \int_{s_i}^{s_{i+1}}\tau(s)T(s_i)\exp{(-\int_{s_i}^{s}\tau(u)\di u)}\di s\\
%	\end{align*}
%\end{center}

\begin{center}
	\begin{align*}
	P_j &= \int_{s_j}^{s_{j+1}}\tau(s)T(s)\,\dif s = \int_{s_j}^{s_{j+1}}\tau(s)\Exp\bracket{-\int_{0}^{s}\tau(u)\dif u}\dif s\\ &=\int_{s_j}^{s_{j+1}}\tau(s)T(s_j)\exp\bracket{-\int_{s_j}^{s}\tau(u)\dif u}\dif s
	=T(s_j)\int_{s_j}^{s_{j+1}}\tau(s)\exp\bracket{-\int_{s_j}^{s}\tau(u)\dif u}\dif s. 
	\end{align*}
\end{center}

\noindent Now, since $\tau$ is a linear function w.r.t. $s$, then the integral $-\int_{s_j}^{s}\tau(u)\dif u$ is a quadratic function w.r.t. $s$. Thus, $P_j$ then becomes an expression of the form $P_j = A\int_{y(s_j)}^{y(s_{j+1})}y\exp(y^2)\dif y$, where $A$ is a constant. Hence, the exact integral can be derived as the simple and closed-form expression:

\begin{equation}
\boxed{
P_j = T(s_j) \cdot \paren{1 - \exp{\bracket{-\frac{(\tau_{j+1}+\tau_j)(s_{j+1}-s_j)}{2}}}}.
}
\label{eq:PMF_linear}
\end{equation}

Moreover, under the piecewise linear opacity assumption, transparency is also derived as the following simple expression:

$$
T(s_j) = \exp\bracket{-\int_0^{s_j} \tau(u)\,\dif u} = \prod_{k=1}^{i} \exp\bracket{-\int_{s_{k-1}}^{s_k}\tau(u)\,\dif u},
$$

\begin{equation}
\boxed{
	T(s_j) = \prod_{k=1}^{i} \exp\bracket{-\frac{(\tau_k+\tau_{k-1})(s_k-s_{k-1})}{2}}.
}
\end{equation}
\vspace{-0.2cm}
\noindent Please see supplement for full detailed derivation.
\vspace{-0.2cm}
% \paragraph{Exact NeRF samples with \emph{continuous} PMF $P_j$.}
\paragraph{Precision Importance Sampling.} Following the same spirit as the derivation for the probability of an interval $P_j$, it also turns out that with our piecewise linear opacity assumption, we are able to derive an exact closed-form solution for inverse transform sampling. Recall that in Sec~\ref{sec:constant_issues}, we pointed the drawback on the CDF $\tilde{F}$ being non-invertible and discontinuous under piecewise constant opacity. We show that this is alleviated in our piecewise linear setting. Concretely, given samples  $s_1, ..., s_N$ resulting in interval probabilities $P_1, ..., P_N$\footnote{We note that DS-NeRF~\cite{kangle2021dsnerf} shows that this will sum to 1 assuming an opaque far plane. $s_{N+1}$ would correspond to the far plane.} from our derivation (Eq~\ref{eq:PMF_linear}), the CDF for \emph{continuous} random variable $t$ is then given as 
% $F(t) = \int_0^t p(s)\dif s = \sum_{s_j<t} P_j + \int_{s_j}^t p(s)\dif s = \sum_{s_j<t} P_j + \int_{s_j}^t \tau(s)T(s)\dif s$. 
\begin{equation}
    F(t) = \int_0^t p(s)\,\dif s = \sum_{s_j<t} P_j + \int_{s_j}^t p(s)\,\dif s = \sum_{s_j<t} P_j + \int_{s_j}^t \tau(s)T(s)\,\dif s
    \label{eq:continuous_cdf}
\end{equation}
Note that unlike in piecewise constant opacity, we don't convert a continuous random variable $s$ to a discrete random variable $\tilde{s}$, thus, the resulting CDF $F$ being continuous. Now, assuming that opacity $\tau \geq 0$ everywhere, from Eq.~\ref{eq:continuous_cdf} we see that $F$ is strictly increasing. Since $F$ is continuous and strictly increasing, then it is invertible. 

Finally, we have our precision importance sampling, where by inverse transform sampling, we can solve for the exact sample $x = F^{-1}(u)$ for $u\sim U(0,1)$ from the given ray distribution $p(s)$ since the CDF $F$ is invertible under piecewise linear opacity. That is, without loss of generality, let sample $u\sim U(0,1)$ fall into the bin $u \in [C_k, C_{k+1}]$, where $C_k = \sum_{j<k}P_j$, which is equivalent to solving for $x\in[s_k, s_{k+1}]$. Reparameterizing $x= s_k + t$, where $t \in [0, s_{k+1}- s_k]$, the exact solution for sample $u$ is given by
\vspace{-0.1cm}
\begin{equation}
\boxed{
    t = \frac{s_{k+1}-s_k}{\tau_{k+1}-\tau_k}\bracket{-\tau_k + \sqrt{\tau_k^2 + \frac{2(\tau_{k+1}-\tau_k)\paren{-\ln \frac{1-u}{T\paren{s_k}}}}{(s_{k+1}-s_k)}}}.
    \label{t_sol_cleaned}
    }
\end{equation}
\vspace{-0.1cm}
Please see supplementary for full derivation. This leads to precisely sampling from the ray distribution $p(s)$ resulting in better importance sampling and stronger depth supervision.
% This leads to the fundamentally correct and exact solution to sampling from the ray distribution $p(s)$ resulting in better importance sampling and stronger depth supervision.
% \vspace{-0.4cm}
% \mika{I'm not sure how to name or position this section. It covers both importance sampling and stronger depth supervision?}
% \mika{where do we say and cite DS-NeRF that it integrates to 1. And do we bring up that for the constant case they normalize -- they don't integrate to 1.} \ke{I think you will first need to point out the non-invertibility of the CDF of a discrete RV, and describe the approximation existing work does to get around the issue. Then you can go over the consequence, i.e, samples being inaccurate when applying inverse transform sampling.}

% Apart from the volume rendering equation, the PMF of the viewing ray is also used to obtain \textbf{samples} from the NeRF  with inverse transform sampling. These samples are then used for different applications such as hierarchical sampling~\cite{} and depth supervision~\cite{}. Concretely by inverse transform sampling, a sample $x$ from the ray distribution is obtain by $x = F^{-1}(u),$ where $u \sim U(0,1)$ and $F(t) = \int_0^t p(s)\dif s = \int_0^t \tau(s)T(s) \dif s$ is the cummulative distribution function (CDF). 

% Given the ray samples $s_1, s_2, ..., s_N$, corresponding PMFs $P_1, P_2, ..., P_N$, we have the CDF of the ray at the samples denoted as $C_j = F(s_j) = \sum_{k<j} P_j$. Under the piecewise constant assumption of opacity, the probability density function $p(s)$, which is approximated by $P_j$ is discontinuous at the bin boundaries, i.e. at the samples, which means that the CDF $F$ is also discontinuous~\ke{This is not quite true - it would be continuous. However, existing work does not do this, and instead take the CDF of the discrete RV} and thus is not invertible which causes a problem whenever samples are draw via inverse transform sampling causing instability. \mika{show a figure here?} Existing works attempt to get around this by shifting and connecting the bin boundaries which is mathematically incorrect \mika{not sure how to say this}~\ke{linear interpolation?}.

% We show that under the piecewise linear assumption on volume density, we are able to mathematically \emph{solve} for the exact sample $x$ corresponding to each $u \sim U(0,1)$ and the solution is unique and always exists. First, we note that under the piecewise linear assumption, $p(s)$ is continuous and hence the CDF $F$ under numerical quadrature is continuous. Without loss of generality, let sample $u\sim U(0,1)$ fall into the bin $u \in [C_k, C_{k+1}]$, then we solve for $x$ such that $x = F^{-1}(u)$:

% Reparameterizing, let $x= s_k + t$, where $t \in [0, s_{k+1}, s_k]$, the exact solution for sample $u$ is given by
% \begin{equation}
% \boxed{
%     t = \frac{(s_{k+1}-s_k)(-\tau_k + \sqrt{\tau_k^2 + \frac{2(\tau_{k+1}-\tau_k)(-\ln \frac{(1-u)}{T(s_k)})}{(s_{k+1}-s_k)}})}{(\tau_{k+1}-\tau_k)}.
%     \label{t_sol_cleaned}
%     }
% \end{equation}


% \begin{center}
%     \begin{align*}
%     u &= \int_0^x T(s)\tau(s)\dif s = \int_0^{s_{k}} T(s)\tau(s)\dif s + \int_{s_{k}}^x T(s)\tau(s)\dif s = c_k + \int_{s_{k}}^x T(s)\tau(s)\dif s\\
%     % &= \int_0^{s_{k}} T(s)\tau(s)\di s + \int_{s_{k}}^x T(s)\tau(s)\di s\\
%     % &= c_k + \int_{s_{k}}^x T(s)\tau(s)\di s\\
%     u - c_k &= \int_{s_{k}}^x T(s)\tau(s)\dif s = \int_{s_{k}}^x \tau(s) T(s_k) \exp{(-\int_{s_k}^x \tau(u) \dif u)}\dif s.\\
%     % &= \int_{s_{k}}^x \tau(s) T(s_k) \exp{(-\int_{s_k}^x \tau(u) \di u)}\di s
%     \end{align*}
% \end{center}

% This leads to a quadratic equation in $x$, where interestingly, we show that a \emph{unique} solution \emph{always exists}. That is, there is always one root such that $x \in [s_k, s_{k+1}]$. Reparameterizing, let $x= s_k + t$, where $t \in [0, s_{k+1}, s_k]$, the exact solution for sample $u$ is given by
% \begin{equation}
% \boxed{
%     t = \frac{(s_{k+1}-s_k)(-\tau_k + \sqrt{\tau_k^2 + \frac{2(\tau_{k+1}-\tau_k)(-\ln \frac{(1-u)}{T(s_k)})}{(s_{k+1}-s_k)}})}{(\tau_{k+1}-\tau_k)}.
%     \label{t_sol_cleaned}
%     }
% \end{equation}

% Please see supplementary for full derivation.
% % and proof that a unique solution $t$, and equivalently $x$, always exists for any $s_k, \tau_k \forall k$ under the condition that $\tau_k \neq \tau_{k+1}$, which would equivalently fall into the constant assumption. 
% This leads to the fundamentally correct and exact solution to sampling from the ray distribution $p(s)$ resulting in better importance sampling and stronger depth supervision.






%%%%%%%%%%%%%%%%%%
% - we derive the exact volumetric rendering equation under th piecewise linear assumption of opacity
% - this leads to a continuous probability distribution along the ray
% - we theoretically show that under this PWL opacity assumption, there is an exact and unique solution to the surface crossing. Leading to correct importance sampling as well as stronger depth supervision.




==> sections/4-results_old.tex <==
% \vspace{-0.3cm}
\section{Results}
\vspace{-0.3cm}
In this section, we present our experimental evaluations to demonstrate the advantages our piecewise linear opacity formulation for volume rendering, which we call \methodname.
\vspace{-0.3cm}
\subsection{Datasets, Evaluation Metrics and Implementation Details.} 
\vspace{-0.3cm}
\paragraph{Datasets and Evaluation Metrics.} We evaluate our method on the standard datasets: Blender and Real Forward Facing datasets as used in~\cite{mildenhall2020nerf}. 
% The Blender dataset contains 8 scenes with camera views placed in a hemisphere at a fixed distance from the object. Real Forward Facing (RFF) is a real-world scene dataset consisting of 8 scenes (5 from LLFF~\cite{mildenhall2019llff} and 3 from NeRF~\cite{mildenhall2020nerf}) captured with a handheld cellphone. 
% We use the released training and test splits for each, where there are 100 training and 200 test images for Blender, while $\frac{1}{8}$ of the images were hold out for testing for Real Forward Facing. 
We use the released training and test splits for each. For dataset details, please see the Supplementary. 
For quantitative comparison, we follow the standard evaluation metrics and report PSNR, SSIM~\cite{wang2004image} and LPIPS~\cite{zhang2018unreasonable} on unseen test views. We also report the root-mean-squared-error (RSME) on the expected ray termination in our depth experiments.
% on the Blender dataset released by the original NeRF~\cite{mildenhall2020nerf} paper. The dataset contains 8 synthetic scenes. We also present results on the standard complex real-world scene dataset, Real Forward Facing, which consists of 8 scenes (5 from LLFF~cite{} and 3 from NeRF~\cite{mildenhall2020nerf}) captured with a handheld cellphone. We use the released training and test splits for each, where there are 100 training and 200 test images for Blender, while $\frac{1}{8}$ of the images were hold out for testing for Real Forward Facing. 
% Furthermore, we constructed a Blender multi-distance benchmark to simulate a more realistic setting where camera captures are at different distances from the object. In contrast, the original Blender scenes contain camera views that are placed in a hemisphere at a \emph{fixed} distance from the object. We instead randomly sample a distance between $[0.5, 1.0]$ of the original hemisphere radius when creating our \textbf{Blender multi-distance} dataset, which is a more realistic setting as one may want to move closer to an object to capture finer details. We use the released data processing pipeline released from~\cite{mildenhall2020nerf} in sampling camera optical axes and additionally sampling a random scaling factor from $U(0.5, 1.0)$ for the camera origin. We note that different from the multi-scale Blender dataset~\cite{barron2021mipnerf}, which varies the camera intrinsics and resolution and does not however change the camera-to-object distance where quadrature is affected ?\mika{Please check this.}. 
% \mika{Finally, we showcase our method on the more challenging real-world datasets (
% mika{unconstrained cameras?}: DTU and Scannet.}

% \mika{For Blender Multi distance, do we want to illustrate that? Ie cameras being closer -- to differentiate from "multi-scale" from mip-nerf.}
% \vspace{-0.4cm}
% \paragraph{Evaluation Metrics.} For quantitative comparison, we follow the standard evaluation metrics and report PSNR, SSIM~\cite{wang2004image} and LPIPS~\cite{zhang2018unreasonable} on unseen test views. We also report the root-mean-squared-error (RSME) on the expected ray termination in our depth experiments.
\vspace{-0.4cm}
\paragraph{Implementation Details.} \methodname is implemented on top of NeRF-Pytorch~\cite{lin2020nerfpytorch}, a reproducible Pytorch implementation of the constant (vanilla)  NeRF, where we simply change the volume rendering to our formulation under piecewise linear opacity and utilize our exact importance sampling derivation. Similar to~\cite{mildenhall2020nerf} we optimize a separate network for the coarse and fine models that are jointly trained with the MSE loss on ground truth images. We use a batch size of 1024 rays and a learning rate of $5\times 10^{-4}$ that decays exponentially to $5\times 10^{-5}$ throughout the course of optimization. We train each scene for 500k iterations which takes $\sim18$ hours on a single Nvidia V100 GPU~\footnote{We rerun and train the vanilla (constant) model using the released reproducible configs from~\cite{lin2020nerfpytorch}.}. Our precision importance sampling enables us to use fewer samples for the fine network, hence keeping the total number of rendering samples the same, we use 128 coarse samples and 64 fine samples to train and test our method. 
% \mika{@Ke please check this sentence.} 
Code will be released upon publication.
\vspace{-0.2cm}
% We use the same architecture as the original NeRF~\cite{mildenhall2020nerf}. \mika{Do I need to say we run constant for the first 2k iterations?} We use a batch size of 1024 rays, Adam optimizer with an initial learning rate of $5\times10^{-4}$ that decays exponentially to $5\times 10^{-5}$ throughout the course of optimization. We train each scene for 500k iterations which takes $\sim18$ hours on a single Nvidia V100 GPU. We reran the original NeRF~\cite{mildenhall2020nerf} piecewise constant baseline also for 500k iterations for fair comparison. We used the released and reproducible implementation from~\cite{lin2020nerfpytorch} fixing a random seed. We build on top of the same codebase \mika{Can I say this?} incorporating the volume rendering equation under piecewise linear density and our precise importance sampling strategy for \methodname~\footnote{Code will be released upon publication.}. Since our approach has more precise importance samples, we use half the number of fine samples compared to the original constant case, which we call refined samples, and instead use more samples for the coarse network for better quadrature approximation. For example, the original NeRF uses 64 coarse and 128 fine samples, our \methodname instead uses 128 coarse samples and 64 fine samples. \footnote{\mika{See supplementary for ablation?}} \mika{@Ke, help here. I'm not sure how to say this.}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{figures/blender_llff_quali_v1.pdf}
    \vspace{-0.4cm}
    \caption{\vspace{-0.5cm}\textbf{Qualitative Results for Blender and Real Forward Facing}.}
    \label{fig:blender_llff}
    \vspace{-0.3cm}
\end{figure}

\input{tables/blender_llff}
\subsection{Experiments on Blender and Real Forward Facing}
% \vspace{-0.3cm}
We first evaluate our \methodname on the standard Blender and Real Forward Facing datasets. Table~\ref{tab:blender_llff} shows that our \methodname (linear) outperforms the vanilla~\cite{mildenhall2020nerf} (constant) model that assumes piecewise constant opacity in all metrics for both the synthetic Blender and Real Forward Facing datasets. Figure~\ref{fig:grazing_angle} and Figure~\ref{fig:blender_llff} show qualitative results. As shown our \methodname is able to achieve sharper textures as shown in the lego's scooper and the bread's surface in the hotdog. Moreover, our approach is also able to recover less fuzzy surfaces as shown in the microphone scene (Figure~\ref{fig:grazing_angle}) where training views are close to the grazing angle of its head. As illustrated, the resulting probability density of the ray corresponding to the marked pixel is peakier than constant as our precision importance sampling allows us to have better samples closer to the surface. We also see clearer ropes in ship, less cloudy interior of the drum, and more solid surfaces such as cleaner leg of the swivel chair in the room scene. 
\vspace{-0.7cm}
% \mika{I'm not sure how to describe the t-rex missing object. Also, there is no chair example of trained on hemis and test on hemis, the chair was on multidist.}

\input{tables/multidist}
\subsection{Experiments on Close-up Views}
\vspace{-0.2cm}
% We further consider a more challenging setting where cameras are moved closer to the objects where details are more apparent. Table~\ref{tab:multidist} (top) shows quantitative results when models are trained on the original hemisphere dataset and tested on different close-up views. Distances 0.25x, 0.5x, 0.75x refer to the scaling factor that is multiplied to original hemisphere radius to obtain new camera origins at different distances from the object. The difficulty of this setting is illustrated as all metrics drop compared to testing only on camera views sampled on the same hemisphere as the training views, where the difficulty increases the closer the camera gets to the object (0.75x to 0.5x to 0.25x). As shown, our \methodname outperforms the vanilla piecewise constant model in all settings and the gap (SSIM and LPIPS) between ours and the constant assumption increases as the setting becomes harder. This is because details become more apparent the closer the camera is to the object needing highlighting the importance of having sharper textures and less fuzzy surfaces.

We further consider the challenging setting of testing on cameras closer to the objects. Table~\ref{tab:multidist} (top) shows quantitative results when training on the original hemisphere dataset and tested on different close-up views. 
% 0.25x, 0.5x, 0.75x refer to the scaling factor that is multiplied to the original radius to obtain new camera origins at different distances from the object. 
As shown by the drop in metrics, the difficulty increases as the camera moves closer to the object (0.75x to 0.5x to 0.25x of the original radius) where details get more apparent. Our \methodname outperforms the vanilla piecewise constant model in all settings and the gap (SSIM and LPIPS) between ours and the constant assumption increases as the setting becomes harder highlighting the importance of recovering shaper texture and less fuzzy surfaces.
% The difficulty of this setting is illustrated as all metrics drop compared to testing only on camera views sampled on the same hemisphere as the training views, where the difficulty increases the closer the camera gets to the object (0.75x to 0.5x to 0.25x). As shown, our \methodname outperforms the vanilla piecewise constant model in all settings and the gap (SSIM and LPIPS) between ours and the constant assumption increases as the setting becomes harder. This is because details become more apparent the closer the camera is to the object needing highlighting the importance of having sharper textures and less fuzzy surfaces.

We also consider the set-up of training with cameras with different distances to the object that result in different sets of ray samples causing conflicts. We generate training views following the data processing pipeline from~\cite{mildenhall2020nerf} with a random distance scaling factor sampled from $U(0.5, 1.0)$. 
% We then train our linear \methodname and the vanilla (constant) model~\cite{mildenhall2020nerf} on this data with multiple camera-to-object distances (Multi Dist) and test on various close-up views. 
As shown in Table~\ref{tab:multidist} (bottom), our \methodname outperforms the vanilla constant baseline in all metrics across different camera distances, where the gap (LPIPS and SSIM) is also larger the closer the camera is to the object, where details are more apparent. The difficulty for the constant (vanilla) case under multiple camera distances is its sensitivity to the choice of samples along the ray. Figure~\ref{fig:conflicting_ray} shows that the conflicting rays cause quadrature instability for under piecewise constant opacity leads to unstable outputs as shown by the noisy texture on the chair. For the constant, the level of noise (gold specs) and blurriness vary at different camera distances, whereas our \methodname renders crisper and more consistent outputs even as the camera is moved closer or further for the object. 

% One can also consider a less constrained set-up on the training views that are collected at various distances from the object. We use the released data processing pipeline from~\cite{mildenhall2020nerf} in sampling camera optical axes and additionally sampling a random scaling factor from $U(0.5, 1.0)$ for the camera origin that is multiplied to the original hemisphere radius. The close-up training cameras in this less constrained setting gives us training views that capture finer details of the object. We then train our linear \methodname and the vanilla (constant) model~\cite{mildenhall2020nerf} on this data with multiple camera-to-object distances (Multi Dist) and test on various close-up views. As shown in Table~\ref{tab:multidist} (bottom), our \methodname outperforms the vanilla constant baseline in all metrics across different camera distances, where the gap (LPIPS and SSIM) is also larger the closer the camera is to the object, where details are more apparent. The difficulty for the piecewise constant assumption under multiple camera distances is its sensitivity to the choice of samples along the ray. As shown in Figure~\ref{fig:conflicting_ray}, the conflicting rays causing quadrature instability for under piecewise constant opacity leads to unstable outputs as shown by the noisy texture on the chair. For the constant assumption, the level of noise (gold specs) and blurriness vary at different camera distances, whereas our \methodname is able to render crisper and more consistent outputs even as the camera is moved closer and further for the object. 
% \mika{@Ke please check these sentences}
\vspace{-0.4cm}
\subsection{Experiments with Depth Supervision}
\vspace{-0.3cm}
\input{tables/depth}We further show that our \methodname enables stronger depth supervision under our piecewise linear opacity assumption due our precision importance sampling that allows for gradients to flow to these more refined samples resulting in more accurate depth. As in previous works~\cite{uy-scade-cvpr23}, we use a sample-based loss for to incorporate depth supervision\footnote{We use the original hyperparameters from~\cite{uy-scade-cvpr23} in this experiment.}. Table~\ref{tab:depth} shows quantitative results when training and testing on the less constrained Blender dataset with cameras at random distances from the object, as described in the previous section, with depth supervision. As shown, our \methodname outperforms the vanilla constant baseline on all metrics including depth RSME demonstrating that our approach allows for stronger depth supervision.





==> sections/5-conclusion_old.tex <==
\section{Conclusion}
  \vspace{-0.2cm}
We proposed a new way to approximate the volume rendering integral that avoids quadrature instability, by considering a piecewise linear approximation to opacity and a piecewise constant approximation to color. We showed that this results in a simple closed-form expression for the integral that is easy to evaluate. We turned this into a new objective for training NeRFs and demonstrated improved rendering quality, more accurate importance sampling and stronger depth supervision. 

% \paragraph{Limitations.}
